Biscotti: A Ledger for Private and Secure Peer-to-Peer Machine Learning

Federated Learning is the current state of the art in supporting secure multi-party machine learning (ML): data is maintained on the owner's device and the updates to the model are aggregated through a secure protocol. However, this process assumes a trusted centralized infrastructure for coordination, and clients must trust that the central service does not use the byproducts of client data. In addition to this, a group of malicious clients could also harm the performance of the model by carrying out a poisoning attack. As a response, we propose Biscotti: a fully decentralized peer to peer (P2P) approach to multi-party ML, which uses blockchain and cryptographic primitives to coordinate a privacy-preserving ML process between peering clients. Our evaluation demonstrates that Biscotti is scalable, fault tolerant, and defends against known attacks. For example, Biscotti is able to protect the privacy of an individual client's update and the performance of the global model at scale when 30% of adversaries are trying to poison the model. The implementation can be found at: https://github.com/DistributedML/Biscotti

==> annotations.tex <==
%% The following is a directive for TeXShop to indicate the main file
%%!TEX root = paper.tex
\usepackage{ifthen}
\usepackage[normalem]{ulem} % for \sout
\usepackage{xcolor}
\usepackage{amssymb}

\newcommand{\ra}{$\rightarrow$}
\newboolean{showedits}
\setboolean{showedits}{true} % toggle to show or hide edits
%\setboolean{showedits}{false} 
\ifthenelse{\boolean{showedits}}
{
	\newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
	\newcommand{\ins}[1]{\textcolor{blue}{\uline{#1}}} % please insert
	\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
	\newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change
}{
	\newcommand{\ugh}[1]{#1} % please rephrase
	\newcommand{\ins}[1]{#1} % please insert
	\newcommand{\del}[1]{} % please delete
	\newcommand{\chg}[2]{#2}
}

\newboolean{showcomments}
\setboolean{showcomments}{false}
%\setboolean{showcomments}{false}
\newcommand{\id}[1]{$-$Id: scgPaper.tex 32478 2010-04-29 09:11:32Z oscar $-$}
\newcommand{\yellowbox}[1]{\fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize#1}}
\newcommand{\triangles}[1]{{\sf\small$\blacktriangleright$\textit{#1}$\blacktriangleleft$}}
\ifthenelse{\boolean{showcomments}}
%{\newcommand{\nb}[2]{{\yellowbox{#1}\triangles{#2}}}
{\newcommand{\nbc}[3]{
 {\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
 {\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}}
 \newcommand{\version}{\emph{\scriptsize\id}}}
{\newcommand{\nbc}[3]{}
 \renewcommand{\ugh}[1]{#1} % please rephrase
 \renewcommand{\ins}[1]{#1} % please insert
 \renewcommand{\del}[1]{} % please delete
 \renewcommand{\chg}[2]{#2} % please change
 \newcommand{\version}{}}
\newcommand{\nb}[2]{\nbc{#1}{#2}{orange}}


\definecolor{ibcolor}{rgb}{0.4,0.6,0.2}
\definecolor{cfcolor}{rgb}{0.2,0.6,0.6}
\definecolor{smcolor}{rgb}{0.8,0.5,0.3}
\definecolor{cycolor}{rgb}{0.0,0.8,0.2}
\newcommand\iv[1]{\nbc{IB}{#1}{ibcolor}}
\newcommand\clem[1]{\nbc{CF}{#1}{cfcolor}}
\newcommand\shayan[1]{\nbc{MS}{#1}{smcolor}}
\newcommand\chris[1]{\nbc{CY}{#1}{smcolor}}

\usepackage{wasysym}
\newcommand\yesml[1]{\nbc{ML {\textcolor{yellow}\sun}}{#1}{mircolor}}

\definecolor{todocolor}{rgb}{0.9,0.1,0.1}
\newcommand\todo[1]{\nbc{TODO}{#1}{todocolor}}


==> background.tex <==
%!TEX root = paper.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Background}
\label{sec:background}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Machine learning (ML) and federated learning.} 
Given a set of training data, a model structure, and a proposed
learning task, ML algorithms \emph{train} an optimal set of
parameters, resulting in a model that optimally performs this task. 
In Biscotti, we assume stochastic gradient descent 
(SGD)~\cite{Bottou:2010} as the optimization algorithm.

In federated learning~\cite{McMahan:2017}, a shared model is updated
through SGD. Each client uses their local training data and their
latest snapshot of the shared model state to compute the optimal update
on the model parameters. The model is then updated and clients update
their local snapshot of the shared model before performing a local
iteration again. The model parameters $w$ are updated at each
iteration $i$ as follows:
\begin{align*}
  w_{i+1} = w_i - \eta_i(\lambda w_i + \frac{1}{b} \sum_{(x_a, y_a)\in
  B_i} \nabla l(w_i, x_a, y_a)) &&&& (1)
\end{align*}
where $\eta_t$ represents a degrading learning rate, $\lambda$ is a
regularization parameter that prevents over-fitting, $B_t$ represents
a gradient batch of local training data examples $(x_i, y_i)$ of size
$b$ and $\nabla l$ represents the gradient of the loss function. 

SGD is a general learning algorithm that can be used to train a variety
of models, including deep learning~\cite{Bottou:2010}. A typical
heuristic involves running SGD for a fixed number of iterations or
halting when the magnitude of the gradient falls below a threshold.
When this occurs, model training is considered complete and the shared
model state $w_t$ is returned as the optimal model $w^*$.

To motivate the multi-party ML setting, federated learning assumes that
clients possess training data that is not identically and independently
distributed (non-IID) across clients. In other works, each client
possesses a subset of the global dataset that contains specific
properties distinct from the global distribution.

To increase privacy guarantees in federated learning, secure
aggregation protocols have been added to the central 
server~\cite{Bonawitz:2017} such that no individual client's update is
directly observable by server or other clients. However, this relies on
a centralized service to perform such an aggregation and does not
provide security against adversarial attacks on ML.

\shayan{Maybe some mention about how equation 1 changes in distributed sgd. All clients compute delta w and then its aggregated together.}

\noindent \textbf{Polynomial Commitments and Verifiable Secret
Sharing}
Polynomial Commitments \cite{Aniket:2010} is a scheme that allows commitments to a 
secret polynomial for verifiable secret sharing \cite{Shamir:1979}.
This allows the committer to distribute secret shares for a secret polynomial among a set
of nodes along with 
witnesses that prove in zero-knowledge that each secret share belongs
to the committed polynomial. The polynomial commitment is constructed
as follows:

Given two groups $G_{1}$ and $G_{2}$ with generators $g_{1}$ and $g_{2}$ of prime order $p$ such that there exists a
asymmetric bilinear pairing $e : G_{1} \times  G_{2} \rightarrow G_{T}$ for which the t-SDH
assumption holds, a commitment public key (PK) is generated such that $ PK = \{g, g^{\alpha}, g^{(\alpha)^{2}}, ..., g^{(\alpha)^{t}}\} \in G_{1}^{t+1}  $ where $\alpha$ is the secret key. The committer can create a commitment to a
polynomial $\phi(x) = \sum_{j=0}^{t} \phi_{j}x^{j} $ of degree $t$ using the commitment PK such that:
\begin{align*}
    	COMM(PK, \phi(x)) = \prod_{j=0}^{deg(\phi)} (g^{\alpha^{j}})^{\phi_{j}}
\end{align*}

Given a polynomial $\phi(x)$ and a commitment $COMM(\phi(x))$, it is
trivial to
verify whether the commitment was generated using the given polynomial
or not. Moreover, we can multiply two commitments to obtain a commitmet to the sum of the polynomials in the commitments by leveraging their homomorphic property: 

\begin{align*}
    	COMM(\phi_{1}(x) + \phi_{2}(x) ) = COMM(\phi_{1}(x)) * COMM(\phi_{2}(x))
\end{align*}


Once the committer has has generated $COMM(\phi(x))$, it can carry out a $(n,t)$
- secret sharing scheme to share the polynomial among a set of $n$
participants in such a way that in the recovery phase a subset of
at least $t$
participants can compute the secret polynomial. All secret shares  
$(i, \phi(i))$ shared with the participants are evaluations of the
polynomial at a unique point $i$
and are accompanied by a commitment to a witness polynomial $COMM(\psi_{i}(x))$ 
 such that $\psi_{i}(x) = \frac{\phi(x) - \phi(i)}{x - i}$. By
 leveraging the
divisibility property of the two polynomials $\{\phi(x),\psi(x)\}$ and the bilinear pairing
function $e$, it is trivial to verify that the secret share comes from the
committed polynomial \cite{Aniket:2010}.

This commitment scheme is unconditionally binding and computationally
hiding
given the Discrete Logarithm assumption holds \cite{Aniket:2010}. This scheme can be
easily extended to provide unconditional hiding by combining it with
another
scheme called Pedersen commitments \cite{Pedersen:1992} however we do
not implement it.  

\clem{Background now feels pretty short, and challenges too long...
I could go into ledgers more: tthe first part of the next section
is too long winded, maybe get right into it and just say we use
ledgers? Removes some of the motivational bits though. I could also
instead get more into adversarial ML as a pre-motivator for ledgers.}

